On Existence of Berk-Nash Equilibria in Misspecified Markov Decision Processes with Infinite Spaces

Model misspecification is a critical issue in many areas of theoretical and empirical economics. In the specific context of misspecified Markov Decision Processes, Esponda and Pouzo (2021) defined the notion of Berk-Nash equilibrium and established its existence in the setting of finite state and action spaces. However, many substantive applications (including two of the three motivating examples presented by Esponda and Pouzo, as well as Gaussian and log-normal distributions, and CARA, CRRA and mean-variance preferences) involve continuous state or action spaces, and are thus not covered by the Esponda-Pouzo existence theorem. We extend the existence of Berk-Nash equilibrium to compact action spaces and sigma-compact state spaces, with possibly unbounded payoff functions. A complication arises because the Berk-Nash equilibrium notion depends critically on Radon-Nikodym derivatives, which are necessarily bounded in the finite case but typically unbounded in misspecified continuous models. The proofs rely on nonstandard analysis and, relative to previous applications of nonstandard analysis in economic theory, draw on novel argumentation traceable to work of the second author on nonstandard representations of Markov processes.

==> myvruler.tex <==
\usepackage{vruler}
\setvruler[10pt][1][1][4][1][20pt][20pt][0pt][\textheight]
\let\orgfillzeros\fillzeros
\def\fillzeros[#1]#2{%
  \begingroup
    \color[rgb]{0.8,0.8,0.8}%
    \orgfillzeros[{#1}]{#2}%
  \endgroup
}


==> novruler.tex <==
% nothing here

